Analysis of Spatial and Spatiotemporal Anomalies Using Persistent Homology: Case Studies with COVID-19 Data

We develop a method for analyzing spatial and spatiotemporal anomalies in geospatial data using topological data analysis (TDA). To do this, we use persistent homology (PH), which allows one to algorithmically detect geometric voids in a data set and quantify the persistence of such voids. We construct an efficient filtered simplicial complex (FSC) such that the voids in our FSC are in one-to-one correspondence with the anomalies. Our approach goes beyond simply identifying anomalies; it also encodes information about the relationships between anomalies. We use vineyards, which one can interpret as time-varying persistence diagrams (which are an approach for visualizing PH), to track how the locations of the anomalies change with time. We conduct two case studies using spatially heterogeneous COVID-19 data. First, we examine vaccination rates in New York City by zip code at a single point in time. Second, we study a year-long data set of COVID-19 case rates in neighborhoods of the city of Los Angeles.

==> TDA covid arxiv resubmission/shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Packages that Abby added
\usepackage{xcolor}
% \usepackage[ruled,vlined]{algorithm2e}
%\usepackage{algorithm}
\usepackage{amsmath, amssymb}
\usepackage{mathtools}
\usepackage{commath}
\usepackage{subfig}
\usepackage[export]{adjustbox}
% \usepackage{subcaption}
\usepackage{multicol}
\usepackage{vwcol}
\usepackage{tikz-cd}
\usepackage{listings}
\usepackage{hyperref}
\usepackage{bm}
\usepackage{cite}
\usepackage{enumitem}
\usepackage{rotating}
\makeatletter
\def\namedlabel#1#2{\begingroup
    #2%
    \def\@currentlabel{#2}%
    \phantomsection\label{#1}\endgroup
}
\makeatother

\newcommand{\creflastconjunction}{, and~}

% Commands that Abby added
%\SetKw{KwTo}{to}
%\SetKwInOut{Input}{input}
%\SetKwInOut{Output}{output}
\newcommand{\scom}{simplicial complex}
\newcommand{\K}{\mathcal{K}}
\newcommand{\intr}{\textnormal{int}}

%%%%%

\newcommand{\map}{\textcolor{blue}}
\newcommand{\abby}{\textcolor{red}}


% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Analysis of {Spatial and} Spatiotemporal Anomalies Using PH}{A. Hickok, D. Needell, and M. A. Porter}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Analysis of {Spatial and} Spatiotemporal Anomalies Using Persistent Homology: Case Studies with COVID-19 Data
\thanks{Submitted to the editors on 26 July 2021.
\funding{AH and MAP acknowledge support from the National Science Foundation (grant number 1922952) through the Algorithms for Threat Detection (ATD) program. MAP also acknowledges support from the National Science Foundation (grant number DMS-2027438) through the RAPID program.}} {DN acknowledges support from the National Science Foundation (grant number DMS-2011140).}}

% Authors: full names plus addresses.
\author{Abigail Hickok\thanks{Department of Mathematics, University of California, Los Angeles, CA, USA
  (\email{ahickok@math.ucla.edu},
  \email{deanna@math.ucla.edu},
  \email{mason@math.ucla.edu}).}
\and Deanna Needell\footnotemark[2]
\and Mason A. Porter\footnotemark[2],\thanks{Santa Fe Institute, Santa Fe, NM, USA}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%% Added on Overleaf: enabling xr
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

% Algorithm environment with page breaks (https://tex.stackexchange.com/questions/33866/algorithm-tag-and-page-break)
\makeatletter
\newenvironment{breakablealgorithm}
  {% \begin{breakablealgorithm}
   \begin{center}
     \refstepcounter{algorithm}% New algorithm
     \hrule height.8pt depth0pt \kern2pt% \@fs@pre for \@fs@ruled
     \renewcommand{\caption}[2][\relax]{% Make a new \caption
       {\raggedright\textbf{\fname@algorithm~\thealgorithm} ##2\par}%
       \ifx\relax##1\relax % #1 is \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##2}%
       \else % #1 is not \relax
         \addcontentsline{loa}{algorithm}{\protect\numberline{\thealgorithm}##1}%
       \fi
       \kern2pt\hrule\kern2pt
     }
  }{% \end{breakablealgorithm}
     \kern2pt\hrule\relax% \@fs@post for \@fs@ruled
   \end{center}
  }
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE
%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

